A unified fourth-order Bhatnagar-Gross-Krook lattice Boltzmann model for high-dimensional linear hyperbolic equations

In this work, we first develop a unified Bhatnagar-Gross-Krook lattice Boltzmann (BGK-LB) model for the $d$($d\geq 1$)-dimensional linear hyperbolic equation (L-HE), where the natural moments and the D$d$Q$(2d^2+1)$ [($2d^2+1$) discrete velocities in $d$-dimensional space] lattice structure are considered. Subsequently, at the acoustic scaling, we conduct an accuracy analysis on the developed BGK-LB model by the direct Taylor expansion (DTE) method, and present the second- and third-order moments of the equilibrium distribution functions (EDFs) to ensure that the BGK-LB model can be fourth-order consistent with the L-HE. And on this basis, when considering the Dirichlet boundary condition, the fourth-order full-way and half-way boundary schemes are proposed to approximate the unknown distribution functions to ensure that the BGK-LB model can be overall fourth-order accurate. Thereafter, based on the kinetic entropy theory, we derive the conditions that the fourth-order moments of the EDFs should satisfy to ensure the microscopic entropy stability of the BGK-LB model. In addition, with the aid of the von Neumann stability analysis, we also discuss the $L^2$ stability of the BGK-LB model and numerically plot the stability regions. In particular, from a numerical perspective, we find that the region of microscopic entropy stability is identical to that of $L^2$ stability. Finally, we carry out some numerical experiments to test the accuracy and stability of the BGK-LB model, and the numerical results are in agreement with our theoretical analysis. In addition, we compare the developed full-way and half-way boundary schemes for the Dirichlet boundary condition, which shows that the full-way boundary scheme is more stable.

==> reference.tex <==





@article{Konstantin2007,
	title={Burgers turbulence},
	author={ J{\'e}r{\'e}mie, B. and Konstantin, K.},
	journal={Phys. Rep.},
	volume={447}, 
	pages={1-66},
	year={2007},
	publisher={Elsevier}
}


@article{Bogaevsky1990,
	title={Inertial dynamics of air bubbles crossing a horizontal fluid--fluid interface},
	author={Bonhomme, R. and Magnaudet, J. and Duval, F. and Piar, B.},
	journal={J. Fluid Mech.},
	volume={707},
	pages={405-443},
	year={2012},
	publisher={Cambridge University Press}
}

@article{Reyna1995,
	title={On the exponentially slow motion of a viscous shock},
	author={Reyna, L. G. and Ward, M. J.},
	journal={Commun. Pure Appl. Math.},
	volume={48},
	number={2},
	pages={79-120},
	year={1995},
	publisher={Wiley Online Library}
}


@article{Buzzicotti2016,
	title={Intermittency in fractal Fourier hydrodynamics: Lessons from the Burgers equation},
	author={Buzzicotti, M. and Biferale, L. and Frisch, U. and Ray, S. S.},
	journal={Phys. Rev. E},
	volume={93},
	number={3},
	pages={033109},
	year={2016},
	publisher={APS}
}



@article{Lighthill1956,
	title={Viscosity effects in sound waves of finite amplitude},
	author={Lighthill, M. J.},
	journal={Surveys in mechanics},
	volume={250351},
	year={1956},
	publisher={Cambridge University Press Cambridge}
}




@article{Nagatani2002,
	title={The physics of traffic jams},
	author={Nagatani, T.},
	journal={Rep. Prog. Phys.},
	volume={65},
	number={9},
	pages={1331},
	year={2002},
	publisher={IOP Publishing}
}


@article{Crighton1979,
	title={Model equations of nonlinear acoustics},
	author={Crighton, D. G.},
	journal={Annu. Rev. Fluid Mech.},
	volume={11},
	number={1},
	pages={11-33},
	year={1979},
	publisher={Annual Reviews 4139 El Camino Way, PO Box 10139, Palo Alto, CA 94303-0139, USA}
}


@article{Bahadir1999,
	title={Numerical solution for one-dimensional Burgers' equation using a fully implicit finite-difference method},
	author={Bahadir, A. R.},
	journal={Int. J. Appl. Math.},
	volume={1},
	number={8},
	pages={897-910},
	year={1999},
	publisher={ACADEMIC PUBLICATIONS}
}



@article{Liao2008,
	title={An implicit fourth-order compact finite difference scheme for one-dimensional Burgers’ equation},
	author={Liao, W. Y.},
	journal={Appl. Math. Comput.},
	volume={206},
	number={2},
	pages={755-764},
	year={2008},
	publisher={Elsevier}
}



@article{Liao2010,
	title={A fourth-order finite-difference method for solving the system of two-dimensional Burgers' equations},
	author={Liao, W. Y},
	journal={Int. J. Numer. Methods Fluids},
	volume={64},
	number={5},
	pages={565-590},
	year={2010},
	publisher={Wiley Online Library}
}



@article{Gao2016,
	title={On a finite difference scheme for Burgers’ equation},
	author={Pandey, K. and Verma, L. and Verma, A. K.},
	journal={Appl. Math. Comput.},
	volume={215},
	number={6},
	pages={2206-2214},
	year={2009},
	publisher={Elsevier}
}


@article{Pandey2009,
	title={On a finite difference scheme for Burgers’ equation},
	author={Pandey, Kanti and Verma, Lajja and Verma, Amit K},
	journal={Appl. Math. Comput.},
	volume={215},
	number={6},
	pages={2206-2214},
	year={2009},
	publisher={Elsevier}
}

@article{Gao2016,
	title={A high-order finite volume method for solving one-dimensional convection and diffusion equations},
	author={Pan, D.},
	journal={Numeri. Heat Tr. B-Fundnumericals},
	volume={71},
	number={6},
	pages={533-548},
	year={2017},
	publisher={Taylor \& Francis}
}



@book{Guo2013,
	title={Lattice Boltzmann method and its application in engineering},
	author={Guo, Z. L and Shu, C.},
	volume={3},
	year={2013},
	publisher={World Scientific}
}


@article{Kruger2017,
	title={The lattice Boltzmann method: principles and practice},
	author={Kr{\"u}ger T. and Kusumaatmaja, H. and Kuzmin, A. and Shardt, O. and Silva, G. and Viggen, E.},
	journal={Cham, Switzerland: Springer International Publishing AG},
	year={2016}
}


@article{Wang2019,
	title={A brief review of the phase-field-based lattice Boltzmann method for multiphase flows},
	author={Wang, H. L. and Yuan, X. L. and Liang, H. and Chai, Z. H. and Shi, B. C.},
	journal={Capillarity},
	volume={2},
	number={3},
	pages={33-52},
	year={2019}, 
}

@book{Succi2008,
	title={The lattice Boltzmann equation: for fluid dynamics and beyond},
	author={Succi, S.},
	year={2001},
	publisher={Oxford university press}
}


@article{Boghosian2004,
	title={Entropic lattice Boltzmann model for Burgers's equation},
	author={Boghosian, Bruce M and Love, Peter and Yepez, Jeffrey},
	journal={Phil. Trans. Roy. Soc. Lon. A},
	volume={362},
	number={1821},
	pages={1691-1701},
	year={2004},
	publisher={The Royal Society}
}


@article{Ma2005,
	title={A new lattice Boltzmann model for solving the coupled viscous Burgers’ equation},
	author={Lai, Huilin and Ma, Changfeng},
	journal={Physica A},
	volume={395},
	pages={445-457},
	year={2014},
	publisher={Elsevier}
}

@article{Zene2005,
	title={Mass transport theory for the Toda lattices, dispersive and dissipative},
	author={Horii, Zene},
	journal={Physica A},
	volume={350},
	number={2-4},
	pages={349-378},
	year={2005},
	publisher={Elsevier}
}


@article{Elton1996,
	title={Comparisons of lattice Boltzmann and finite difference methods for a two-dimensional viscous Burgers equation},
	author={Elton, Bracy H},
	journal={SIAM J. Sci. Comput.},
	volume={17},
	number={4},
	pages={783-813},
	year={1996},
	publisher={SIAM}
}


@article{Velivelli2006,
	title={Parallel performance and accuracy of lattice Boltzmann and traditional finite difference methods for solving the unsteady two-dimensional Burger's equation},
	author={Velivelli, AC and Bryden, KM},
	journal={Physica A},
	volume={362},
	number={1},
	pages={139-145},
	year={2006},
	publisher={Elsevier}
} 

@article{Duan2006,
	title={Lattice Boltzmann model for two-dimensional unsteady Burgers’ equation},
	author={Duan, YaLi and Liu, RuXun},
	journal={J. Comput. Appl. Math.},
	volume={206},
	number={1},
	pages={432--439},
	year={2007},
	publisher={Elsevier}
}


@article{Zhang2008,
	title={Lattice Boltzmann method for one and two-dimensional Burgers equation},
	author={Zhang, Jianying and Yan, Guangwu},
	journal={Physica A},
	volume={387},
	number={19-20},
	pages={4771-4786},
	year={2008},
	publisher={Elsevier}
}



@article{Li2018,
	title={Lattice Boltzmann models for two-dimensional coupled Burgers’ equations},
	author={Li, Qianhuan and Chai, Zhenhua and Shi, Baochang},
	journal={Comput. Math. Appl.},
	volume={75},
	number={3},
	pages={864-875},
	year={2018},
	publisher={Elsevier}
}


@article{Chai2008,
	title={A unified lattice Boltzmann model for some nonlinear partial differential equations},
	author={Chai, Zhenhua and Shi, Baochang and Zheng, Lin},
	journal={Chaos, Solitons Fract.},
	volume={36},
	number={4},
	pages={874--882},
	year={2008},
	publisher={Elsevier}
}


@article{Chai2014,
	title={Lattice Boltzmann model for high-order nonlinear partial differential equations},
	author={Chai, Zhenhua and He, Nanzhong and Guo, Zhaoli and Shi, Baochang},
	journal={Phys. Rev. E},
	volume={97},
	number={1},
	pages={013304},
	year={2018},
	publisher={APS}
}


@article{Qi2018,
	title={Cole-Hopf Transformation Based Lattice Boltzmann Model for One-dimensional Burgers’ Equation},
	author={Qi, Xiao-Tong and Shi, Bao-Chang and Chai, Zhen-Hua},
	journal={Commun. Theor. Phys.},
	volume={69},
	number={3},
	pages={329},
	year={2018},
	publisher={IOP Publishing}
}

@article{Rong2023,
	title={A lattice Boltzmann model based on Cole-Hopf transformation for N-dimensional coupled Burgers' equations},
	author={Rong, Fumei and Li, Qianhuan and Shi, Baochang and Chai, Zhenhua},
	journal={Comput. Math. Appl.},
	volume={134},
	pages={101-111},
	year={2023},
	publisher={Elsevier}
}


@article{cole1951,
	title={On a quasi-linear parabolic equation occurring in aerodynamics},
	author={Cole, Julian D},
	journal={Q. App. Math.},
	volume={9},
	number={3},
	pages={225-236},
	year={1951}
}


@article{Yang2019,
	title={The Sinc-Galerkin methods of the Burgers' equation based on the Hopf-Cole transformation},
	author={Mei, Yang and Fengqun, Zhao and Chong, Guo},
	journal={Chin. J. Comput. Mech.},
	year={2019}
}

@article{Mitta2009,
	title={Differential quadrature method for two-dimensional Burgers' equations},
	author={Mittal, RC and Jiwari, Ram},
	journal={Int. J. Comput. Meth. En.},
	volume={10},
	number={6},
	pages={450-459},
	year={2009},
	publisher={Taylor \& Francis}
}


@article{Anikonov2015,
	title={The Hopf-Cole transformation and multidimensional representations of solutions to evolution equations},
	author={Anikonov, Yu E and Ayupova, NB},
	journal={J. Appl. Ind. Math.},
	volume={9},
	number={1},
	pages={11},
	year={2015},
	publisher={Springer Nature BV}
}


@article{Zhao2011,
	title={The new numerical method for solving the system of two-dimensional Burgers’ equations},
	author={Zhao, Guozhong and Yu, Xijun and Zhang, Rongpei},
	journal={Comput. Math. Appl.},
	volume={62},
	number={8},
	pages={3279-3291},
	year={2011},
	publisher={Elsevier}
}


@article{Mukundan2019,
	title={Multistep methods for the numerical simulation of two-dimensional Burgers’ equation},
	author={Mukundan, Vijitha and Awasthi, Ashish and Aswin, VS},
	journal={Differ. Equ. Dyn. Syst.},
	pages={1-24},
	year={2019},
	publisher={Springer}
}


@article{Zhanlav2016,
	title={Higher-order numerical solution of two-dimensional coupled Burgers’ equations},
	author={Zhanlav, T and Chuluunbaatar, O and Ulziibayar, V},
	journal={Am. J. Comput. Math.},
	volume={6},
	number={02},
	pages={120-129},
	year={2016}
}


@article{Ginzburg2002,
	title={Multiple--relaxation--time lattice Boltzmann models in three dimensions},
	author={d'Humi{\`e}res, Dominique},
	journal={Phil. Trans. R. Soc. Lond.   A },
	volume={360},
	number={1792},
	pages={437-451},
	year={2002},
	publisher={The Royal Society}
}


@article{Chai2020,
	title={Multiple-relaxation-time lattice Boltzmann method for the Navier-Stokes and nonlinear convection-diffusion equations: Modeling, analysis, and elements},
	author={Chai, Zhenhua and Shi, Baochang and others},
	journal={Phys. Rev. E},
	volume={102},
	number={2},
	pages={023306},
	year={2020},
	publisher={APS}
}



@article{Chai2023,
	title={Rectangular multiple-relaxation-time lattice Boltzmann method for the Navier-Stokes and nonlinear convection-diffusion equations: General equilibrium and some important issues},
	author={Chai, Zhenhua and Yuan, Xiaolei and Shi, Baochang and others},
	journal={Phys. Rev. E},
	volume={108},
	number={1},
	pages={015304},
	year={2023},
	publisher={APS}
}


@article{Ginzburg2005,
	title={Equilibrium-type and link-type lattice Boltzmann models for generic advection and anisotropic-dispersion equation},
	author={Ginzburg, Irina},
	journal={Adv. Water Resour.},
	volume={28},
	number={11},
	pages={1171-1195},
	year={2005},
	publisher={Elsevier}
}


@article{Lallemand2000,
	title={Theory of the lattice Boltzmann method: Dispersion, dissipation, isotropy, Galilean invariance, and stability},
	author={Lallemand, Pierre and Luo, Li-Shi},
	journal={Phys. Rev. E},
	volume={61},
	number={6},
	pages={6546},
	year={2000},
	publisher={APS}
}



@article{Pan2006,
	title={An evaluation of lattice Boltzmann schemes for porous medium flow simulation},
	author={Pan, Chongxun and Luo, Li-Shi and Miller, Cass T},
	journal={Comput. Fluids},
	volume={35},
	number={8-9},
	pages={898-909},
	year={2006},
	publisher={Elsevier}
}


@article{Cui2016,
	title={Discrete effect on the halfway bounce-back boundary condition of multiple-relaxation-time lattice Boltzmann model for convection-diffusion equations},
	author={Cui, Shuqi and Hong, Ning and Shi, Baochang and Chai, Zhenhua},
	journal={Phys. Rev. E},
	volume={93},
	number={4},
	pages={043311},
	year={2016},
	publisher={APS}
} 


@article{Luo2011,
	title={Numerics of the lattice Boltzmann method: Effects of collision models on the lattice Boltzmann simulations},
	author={Luo, Li-Shi and Liao, Wei and Chen, Xingwang and Peng, Yan and Zhang, Wei and others},
	journal={Phys. Rev. E},
	volume={83},
	number={5},
	pages={056710},
	year={2011},
	publisher={APS}
}

@article{Yu2023,
	title={A multiple-relaxation-time lattice Boltzmann model for Burgers equation},
	author={Yu, Xiaomei and Zhang, Ling and Hu, Beibei and Hu, Ye},
	journal={Math. Methods   Appl. Sci.},
	year={2023},
	publisher={Wiley Online Library}
}


@article{Suga,
	title={An accurate multi-level finite difference scheme for 1D diffusion equations derived from the lattice Boltzmann method},
	author={Suga, Shinsuke},
	journal={J. Stat. Phys.},
	volume={140},
	pages={494-503},
	year={2010},
	publisher={Springer}
}	

@article{Lin2022,
	title={Multiple-relaxation-time lattice Boltzmann model-based four-level finite-difference scheme for one-dimensional diffusion equations},
	author={Lin, Yuxin and Hong, Ning and Shi, Baochang and Chai, Zhenhua},
	journal={Phys. Rev. E},
	volume={104},
	number={1},
	pages={015312},
	year={2021},
	publisher={APS}
}



@article{Chen2023,
	title={A general fourth-order mesoscopic multiple-relaxation-time lattice Boltzmann model and equivalent macroscopic finite-difference scheme for two-dimensional diffusion equations},
	author={Chen, Ying and Chai, Zhenhua and Shi, Baochang},
	journal={arXiv preprint arXiv:2308.05280},
	year={2023}
}


@article{Be2023,
	title={Finite Difference formulation of any lattice Boltzmann scheme},
	author={Bellotti, Thomas and Graille, Benjamin and Massot, Marc},
	journal={Numer. Math.},
	volume={152},
	number={1},
	pages={1-40},
	year={2022},
	publisher={Springer}
}

@article{Chen2023-GP,
	title={The macroscopic finite-difference scheme and modified equations of the general propagation multiple-relaxation-time lattice Boltzmann model},
	author={Chen, Ying and Liu, Xi and Chai, Zhenhua and Shi, Baochang},
	journal={arXiv preprint arXiv:2308.11882},
	year={2023}
}




